Targeted Supervised Contrastive Learning for Long-Tailed Recognition

Real-world data often exhibits long tail distributions with heavy class imbalance, where the majority classes can dominate the training process and alter the decision boundaries of the minority classes. Recently, researchers have investigated the potential of supervised contrastive learning for long-tailed recognition, and demonstrated that it provides a strong performance gain. In this paper, we show that while supervised contrastive learning can help improve performance, past baselines suffer from poor uniformity brought in by imbalanced data distribution. This poor uniformity manifests in samples from the minority class having poor separability in the feature space. To address this problem, we propose targeted supervised contrastive learning (TSC), which improves the uniformity of the feature distribution on the hypersphere. TSC first generates a set of targets uniformly distributed on a hypersphere. It then makes the features of different classes converge to these distinct and uniformly distributed targets during training. This forces all classes, including minority classes, to maintain a uniform distribution in the feature space, improves class boundaries, and provides better generalization even in the presence of long-tail data. Experiments on multiple datasets show that TSC achieves state-of-the-art performance on long-tailed recognition tasks.

==> source/intro-1.tex <==
\section{Introduction}
% Contrastive learning has been popularly explored as it can learn data representations without requiring manual annotations and offer attractive potential of leveraging the vast amount of unlabeled data in the wild to obtain strong representation models \cite{xxx}. Contrastive learning learns representations on a hypersphere by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset. Recently, the supervised version of contrastive learning \cite{xxx} also demonstrates superior performance on image classification datasets. With the class information provided by the label, supervised contrastive learning choose positive samples as those samples of the same class. 

% Self-supervised learning has become a prevalent choice to extract information from unlabeled data sources, without any manual annotations~\cite{oord2018representation, doersch2015unsupervised, noroozi2016unsupervised, gidaris2018unsupervised}. 
% In recent years, a resurgence of work in contrastive learning~\cite{he2020momentum, chen2020simple, chen2021exploring, khosla2020supervised, wang2020understanding, li2020making, grill2020bootstrap} has led to major advances in self-supervised representation learning. 
% Contrastive learning learns representations on a hypersphere by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset.
% % During training, contrastive learning learns representations on a hypersphere by attracting the positive samples and repulsing the negative samples~\cite{wang2020understanding}. 
% Recently, supervised contrastive learning (SupCon)~\cite{khosla2020supervised} leverages the class label information into the selection of positive and negative samples and extend contrastive learning to supervised setting, achieving superior performance than the cross-entropy counterpart~\cite{graf2021dissecting}.

% However, most existing contrastive learning methods focus on learning data representations from the artificially balanced datasets, e.g. ImageNet \cite{xxx}, where all classes have almost the same number of training data. But in reality, real-world data are often long-tail distributed over semantic classes: A few classes contain many
% instances, whereas most classes contain only a few instances. Such imbalanced datasets are very challenging for supervised learning methods, leading to noticeable performance drop \cite{xxx}. Prior works typically preventing the many head-class instances from overwhelming the few tail-class instances by class re-balancing/re-weighting which gives more importance
% to tail instances \cite{xxx}. \cite{kang2020exploring} is the first attempt to investigate the potential of supervised contrastive learning on dataset with long-tail distribution. It applies supervised contrastive learning on several datasets with long-tail distribution and achieves good performances.

Real-world data often have a long-tail distribution over classes: A few classes contain many instances (head classes), whereas most classes contain only a few instances (tail classes). For example, in the task of natural species classification \cite{van2018inaturalist}, the training data is highly imbalanced because some species are common while some are rare, while all species are of same importance during testing. The task of long-tailed recognition is defined on datasets with long-tail distribution over classes in training set and with uniform distribution over classes in test set. Neural networks trained on such data typically favor the head classes, leading to poor performances on the tail classes \cite{ando2017deep, buda2018systematic, collobert2008unified, yang2019me}. Previous techniques, such as data re-sampling strategies~\cite{chawla2002smote, shen2016relay, buda2018systematic, ando2017deep} or designing class-imbalanced loss~\cite{cao2019learning, cui2019class, dong2018imbalanced, khan2019striking, khan2017cost, byrd2019effect}, have been focused on preventing head classes from overwhelming the tail classes. 
% Recently, ~\cite{kang2019decoupling, zhou2020bbn} decouples representation learning from classifier learning and suggests the promise of pre-training a feature extractor to learn good feature space. ~\cite{yang2020rethinking} for the first time introduces a self-supervised pre-training as initialization to alleviate the imbalanced label bias issue.
Recently, KCL \cite{kang2020exploring} first investigates the potential of supervised contrastive loss with long-tailed label distributions. Instead of taking all samples with the same class \textcolor{red}{in a batch} as positives, it constantly samples $k$ positive for each data point, so the number of positive samples are balanced for instances from different classes. 

\begin{figure}[t]
\begin{center}
%\includegraphics[width=\linewidth]{pos-neg}
%\vspace{-15pt}
\label{fig:intro_rf}
\includegraphics[width=0.48\textwidth]{teaser} 
\end{center}
\vspace{-10pt}
\caption{\footnotesize{
%(a) In human pose estimation, identity information could serve as shortcut to pose features. 
Feature distribution of Supervised contrastive learning and \name~on three classes of CIFAR10.}}
\label{fig:intro1}
\vspace{-10pt}
\end{figure}

It is widely known that contrastive loss achieves superior performances by promoting both the \textit{alignment} and \textit{uniformity} of the feature space \cite{wang2020understanding,graf2021dissecting}. Intuitively, better alignment indicates smaller distance between samples within the same class, while better uniformity indicates larger distance between different classes which brings clearer decision boundaries between classes. However, \cite{kang2020exploring} only focuses on balancing the number of positive samples for each class on long-tailed dataset to improve alignment, but ignore the detrimental effect of imbalanced distribution on uniformity. 

Fig.~\ref{fig:intro1} shows the feature space over three classes of training instances with KCL \cite{kang2020exploring} on CIFAR-10. When the training data is balanced, the feature distribution of KCL is also balanced. However, as the training data become imbalanced, the classes with fewer training instances starts to collapse with each other, leading to unclear and inseparable decision boundaries between classes, and thus deteriorate the classification performance. This is because the imbalanced data distribution naturally puts more weights on the uniformity loss between head class and tail class and less weights on that between two tail classes, making the distance between head and tail classes much larger than the distance between two tail classes. As a result, the more imbalanced the long-tailed data, the more biased and less uniformly distributed the feature space. 


% However, this first attempt does not specifically design the contrastive loss for the long-tailed distribution of the dataset. As shown in Fig. \ref{fig:intro1} (a), classes with fewer training instances could collapse with other classes with similar semantics, resulting in unclear decision boundaries between classes and poor classification performance. This is because similar to cross entropy (CE) loss, the imbalanced data distribution naturally puts more weights on the supervised contrastive (SC) loss of major classes and less weights on that of minor classes. As a result, the feature distribution learned by simply applying SC loss to long-tailed dataset can be both imbalanced and not uniformly distributed, as also shown in Fig. \ref{fig:intro2}.

% In order to further tackle the data imbalance challenge, it is  vital to understand the geometric arrangement of feature space at minimal supervised contrastive (SC) loss on balanced and imbalanced datasets. 

% \begin{figure*}
% \begin{center}
% %\includegraphics[width=\linewidth]{pos-neg}
% %\vspace{-15pt}
% \begin{tabular}{ccccc}
% % \includegraphics[width=0.14\textwidth]{mpii2.png} & \hspace*{-0.12in}
% \label{fig:intro_rf}
% \includegraphics[width=0.18\textwidth]{teaser2-1} & 
% \includegraphics[width=0.18\textwidth]{teaser2-2} & 
% \includegraphics[width=0.18\textwidth]{teaser2-3} & 
% \includegraphics[width=0.18\textwidth]{teaser2-4} & 
% \includegraphics[width=0.18\textwidth]{teaser2-5}\\
% % {\footnotesize (a) Pose Estimation} & \hspace*{-0.12in}
% {\footnotesize (a) $\rho=1:1:1$} & \hspace*{0.13in} {\footnotesize (b) $\rho=1:1:10$} & \hspace*{0.13in} {\footnotesize (c) $\rho=1:1:100$} & \hspace*{0.13in} {\footnotesize (d) $\rho=1:10:100$} & \hspace*{0.13in} {\footnotesize (e) $\rho=1:100:100$}
% \end{tabular}
% \end{center}
% \vspace{-10pt}
% \caption{\footnotesize{
% %(a) In human pose estimation, identity information could serve as shortcut to pose features. 
% Feature distribution learned by SC loss on a synthetic 3-classes dataset with different imbalanced ratio $\rho$ for each class. Each solid dot denotes the feature learned for each class. Imbalanced data distribution can cause the feature distribution to be imbalanced.}}
% \label{fig:intro2}
% \vspace{-10pt}
% \end{figure*}

% Ideally, we want the feature distribution to be like Fig. \ref{fig:intro1} (b), where the class centers are uniformly distributed on the hypersphere. One natural solution is to perform class-balanced sampling or class re-weighting during training. However, as shown in \cite{kang2019decoupling}, class re-balancing and class re-weighting could harm the quality of the learned representation. Therefore, we want a training strategy that performs instance-balanced sampling over the long-tailed dataset, while still be able to learn a balanced and uniform feature space. 

Ideally, since the test set of long-tailed recognition task is balanced, the feature space should be also balanced where the class centers are uniformly distributed on the hypersphere and thus allows clearer inter-class decision boundaries. One possible solution is to take data-balanced sampling or class re-weighting techniques during contrastive training. However, these techniques are not good for representation learning. As shown in~\cite{kang2019decoupling}, these techniques improve tail classes performance at the cost of head classes performance and could harm the quality of the learned features. 
Therefore, a method that performs instance-balanced sampling while still be able to learn a uniform feature space is needed. 

% To solve this problem, in this paper, we propose targeted supervised contrastive learning for long-tailed recognition. Instead of letting the network learn where the class should stay by itself, we precompute the optimal location of each class center and assign them to each instance of the same class during training.  We then propose a targeted contrastive loss to leverage the assigned targets into contrastive loss by regarding the target as an additional positive sample of each class, improving the uniformity of the learned representations. Moreover, to make reasonable assignment for each class, we propose an online matching training scheme that adaptively matches samples from each class to targets during training, and thus preserves the semantic structure of the learned representation.

In this paper, we propose targeted supervised contrastive learning (\name) for long-tailed recognition. To avoid the feature space being dominated and biased by the head classes during training, we generate the optimal locations of class centers in advance as training targets, which are uniformly distributed on the hypersphere. We further propose an online matching training scheme that adaptively matches samples from each class to targets during training. As shown in Fig. \ref{fig:intro1}, \name~learns a balanced feature space regardless of the  imbalance ratio of training set, hence achieves much better performance than KCL. We further evaluate \name~on several different long-tailed recognition datasets including CIFAR-10-LT, CIFAR-100-LT, ImageNet-LT, and iNaturalist, and achieves the state-of-the-art (SOTA) performances on all of them.

To summarize, the paper makes the following contributions:
\begin{Itemize}
    \item It introduces \name, a novel framework for long-taild recognition problem to avoid the feature space being dominated and biased by the head classes.
    \item It empirically shows that supervised contrastive learning baselines can suffer from poor uniformity on long-tailed recognition problem and thus degrade their performances.
    \item It further shows that \name~achieves SOTA long-tailed recognition performances on multiple datasets, demonstrating the effectiveness of the proposed method.
\end{Itemize}


==> source/intro-old.tex <==
\section{Introduction}
% Contrastive learning has been popularly explored as it can learn data representations without requiring manual annotations and offer attractive potential of leveraging the vast amount of unlabeled data in the wild to obtain strong representation models \cite{xxx}. Contrastive learning learns representations on a hypersphere by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset. Recently, the supervised version of contrastive learning \cite{xxx} also demonstrates superior performance on image classification datasets. With the class information provided by the label, supervised contrastive learning choose positive samples as those samples of the same class. 

% Self-supervised learning has become a prevalent choice to extract information from unlabeled data sources, without any manual annotations~\cite{oord2018representation, doersch2015unsupervised, noroozi2016unsupervised, gidaris2018unsupervised}. 
% In recent years, a resurgence of work in contrastive learning~\cite{he2020momentum, chen2020simple, chen2021exploring, khosla2020supervised, wang2020understanding, li2020making, grill2020bootstrap} has led to major advances in self-supervised representation learning. 
% Contrastive learning learns representations on a hypersphere by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset.
% % During training, contrastive learning learns representations on a hypersphere by attracting the positive samples and repulsing the negative samples~\cite{wang2020understanding}. 
% Recently, supervised contrastive learning (SupCon)~\cite{khosla2020supervised} leverages the class label information into the selection of positive and negative samples and extend contrastive learning to supervised setting, achieving superior performance than the cross-entropy counterpart~\cite{graf2021dissecting}.

% However, most existing contrastive learning methods focus on learning data representations from the artificially balanced datasets, e.g. ImageNet \cite{xxx}, where all classes have almost the same number of training data. But in reality, real-world data are often long-tail distributed over semantic classes: A few classes contain many
% instances, whereas most classes contain only a few instances. Such imbalanced datasets are very challenging for supervised learning methods, leading to noticeable performance drop \cite{xxx}. Prior works typically preventing the many head-class instances from overwhelming the few tail-class instances by class re-balancing/re-weighting which gives more importance
% to tail instances \cite{xxx}. \cite{kang2020exploring} is the first attempt to investigate the potential of supervised contrastive learning on dataset with long-tail distribution. It applies supervised contrastive learning on several datasets with long-tail distribution and achieves good performances.

Real-world data are often long-tail distributed over semantic classes: A few classes contain many instances (head classes), whereas most classes contain only a few instances (tail classes). For critical applications, such as medical diagnosis, autonomous driving, and fairness, the data are by their nature heavily imbalanced, and the minor classes data are in particularly important. Such imbalanced datasets pose major challenges for modern supervised learning frameworks, leading to significant performance drop~\cite{ando2017deep, buda2018systematic, collobert2008unified, yang2019me}. Previous techniques, such as data re-sampling strategies~\cite{chawla2002smote, shen2016relay, buda2018systematic, ando2017deep} or designing class-imbalanced loss~\cite{cao2019learning, cui2019class, dong2018imbalanced, khan2019striking, khan2017cost, byrd2019effect}, have been focused on preventing head class from overwhelming the tail class. 
% Recently, ~\cite{kang2019decoupling, zhou2020bbn} decouples representation learning from classifier learning and suggests the promise of pre-training a feature extractor to learn good feature space. ~\cite{yang2020rethinking} for the first time introduces a self-supervised pre-training as initialization to alleviate the imbalanced label bias issue.
Recently, ~\cite{kang2020exploring} first investigates the potential of supervised contrastive learning with long-tailed label distributions and shows a $k$-positive variant of supervised contrastive loss benefits a lot on several datasets.

\begin{figure}
\begin{center}
%\includegraphics[width=\linewidth]{pos-neg}
%\vspace{-15pt}
\begin{tabular}{cc}
% \includegraphics[width=0.14\textwidth]{mpii2.png} & \hspace*{-0.12in}
\label{fig:intro_rf}
\includegraphics[width=0.22\textwidth]{teaser-sc} & 
\includegraphics[width=0.22\textwidth]{teaser-tsc}\\
% {\footnotesize (a) Pose Estimation} & \hspace*{-0.12in}
{\footnotesize (a) SupCon} & \hspace*{0.13in} {\footnotesize (b) \name}
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{\footnotesize{
%(a) In human pose estimation, identity information could serve as shortcut to pose features. 
Feature distribution of Supervised contrastive learning and \name~on CIFAR10.}}
\label{fig:intro1}
\vspace{-10pt}
\end{figure}

% However, this first attempt does not specifically design the contrastive loss for the long-tailed distribution of the dataset. As shown in Fig. \ref{fig:intro1} (a), classes with fewer training instances could collapse with other classes with similar semantics, resulting in unclear decision boundaries between classes and poor classification performance. This is because similar to cross entropy (CE) loss, the imbalanced data distribution naturally puts more weights on the supervised contrastive (SC) loss of major classes and less weights on that of minor classes. As a result, the feature distribution learned by simply applying SC loss to long-tailed dataset can be both imbalanced and not uniformly distributed, as also shown in Fig. \ref{fig:intro2}.

However, this first attempt to leverage supervised contrastive learning under the imbalanced data setting did not consider the characteristic of imbalanced datasets, and thus suffers from the poor uniformity introduced by data imbalance. 
% In order to further tackle the data imbalance challenge, it is  vital to understand the geometric arrangement of feature space at minimal supervised contrastive (SC) loss on balanced and imbalanced datasets. 
Fig.~\ref{fig:intro1} (a) shows the feature space over 10 classes of training instances with supervised contrastive (SC) loss. The classes with fewer training instances collapse with classes that share similar semantics (e.g. ship and truck), leading to unclear and inseparable decision boundaries between classes, and thus deteriorate the classification performance. Intuitively, similar to learning with cross-entropy (CE) loss, the imbalanced data distribution naturally puts more weights on the SC loss of major classes and less weights on that of minor classes. As a result, the feature space is not uniformly distributed. Fig.~\ref{fig:intro2} visualizes the optimal feature spaces of the balanced and different imbalanced toy datasets with simply applying SC loss. The feature space of a balanced dataset is uniformly distributed on a sphere. However, the more imbalanced the long-tailed data, the more biased and less uniformly distributed the feature space. 

\begin{figure*}
\begin{center}
%\includegraphics[width=\linewidth]{pos-neg}
%\vspace{-15pt}
\begin{tabular}{ccccc}
% \includegraphics[width=0.14\textwidth]{mpii2.png} & \hspace*{-0.12in}
\label{fig:intro_rf}
\includegraphics[width=0.18\textwidth]{teaser2-1} & 
\includegraphics[width=0.18\textwidth]{teaser2-2} & 
\includegraphics[width=0.18\textwidth]{teaser2-3} & 
\includegraphics[width=0.18\textwidth]{teaser2-4} & 
\includegraphics[width=0.18\textwidth]{teaser2-5}\\
% {\footnotesize (a) Pose Estimation} & \hspace*{-0.12in}
{\footnotesize (a) $\rho=1:1:1$} & \hspace*{0.13in} {\footnotesize (b) $\rho=1:1:10$} & \hspace*{0.13in} {\footnotesize (c) $\rho=1:1:100$} & \hspace*{0.13in} {\footnotesize (d) $\rho=1:10:100$} & \hspace*{0.13in} {\footnotesize (e) $\rho=1:100:100$}
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{\footnotesize{
%(a) In human pose estimation, identity information could serve as shortcut to pose features. 
Feature distribution learned by SC loss on a synthetic 3-classes dataset with different imbalanced ratio $\rho$ for each class. Each solid dot denotes the feature learned for each class. Imbalanced data distribution can cause the feature distribution to be imbalanced.}}
\label{fig:intro2}
\vspace{-10pt}
\end{figure*}

% Ideally, we want the feature distribution to be like Fig. \ref{fig:intro1} (b), where the class centers are uniformly distributed on the hypersphere. One natural solution is to perform class-balanced sampling or class re-weighting during training. However, as shown in \cite{kang2019decoupling}, class re-balancing and class re-weighting could harm the quality of the learned representation. Therefore, we want a training strategy that performs instance-balanced sampling over the long-tailed dataset, while still be able to learn a balanced and uniform feature space. 

Ideally, for imbalanced datasets, the feature space should be like Fig.~\ref{fig:intro1} (b), where the class centers are uniformly distributed on the hypersphere and thus allows clearer inter-class decision boundaries. One possible solution is to take data-balanced sampling or class re-weighting techniques during contrastive training. However, these techniques are not good for representation learning. As shown in~\cite{kang2019decoupling}, these techniques improve tail classes performance at the cost of head classes performance and could harm the quality of learned features. 
Therefore, a method that performs instance-balanced sampling while still be able to learn a uniform feature space is needed. 

% To solve this problem, in this paper, we propose targeted supervised contrastive learning for long-tailed recognition. Instead of letting the network learn where the class should stay by itself, we precompute the optimal location of each class center and assign them to each instance of the same class during training.  We then propose a targeted contrastive loss to leverage the assigned targets into contrastive loss by regarding the target as an additional positive sample of each class, improving the uniformity of the learned representations. Moreover, to make reasonable assignment for each class, we propose an online matching training scheme that adaptively matches samples from each class to targets during training, and thus preserves the semantic structure of the learned representation.

In this paper, we propose \name, a targeted supervised contrastive learning method for long-tailed recognition. We first analyze the geographic arrangement that an optimal feature space should be like under the supervised contrastive learning. Based on this analysis, to avoid the feature space dominated and biased by the major classes, we generate the optimal location of each class center in advance and assign it automatically to each instance of the same class during training. Specifically, with the precomputed targets, we propose an online matching training scheme that adaptively matches samples from each class to targets during training, and thus preserves the semantic structure of the learned representation. We then propose a targeted contrastive loss to leverage the assigned targets into contrastive loss by regarding the target as an additional positive sample of each class, improving the uniformity of the learned representations.



We evaluate \name~on several different long-tailed recognition datasets including CIFAR-10-LT, CIFAR-100-LT, ImageNet-LT, and iNaturalist, and achieves the SOTA of single model performance on all those datasets.

To summarize, the paper makes the following contributions:
\begin{Itemize}
    \item It introduces \name, a novel framework for long-taild recognition problem.
    \item It empirically shows that SOTA supervised contrastive learning baselines can suffer from poor uniformity on long-tailed recognition problem, and thus degrade their performances on both major and minor classes.
    \item It further shows that \name~outperforms SOTA long-tailed recognition methods on multiple datasets, demonstrating the effectiveness of the proposed method.
\end{Itemize}

